A hybrid parametric-deep learning approach for sound event localization and detection

This work describes and discusses an algorithm submitted to the Sound Event Localization and Detection Task of DCASE2019 Challenge. The proposed methodology relies on parametric spatial audio analysis for source localization and detection, combined with a deep learning-based monophonic event classifier. The evaluation of the proposed algorithm yields overall results comparable to the baseline system. The main highlight is a reduction of the localization error on the evaluation dataset by a factor of 2.6, compared with the baseline performance.

==> changelog.tex <==
CHANGELOG - WORKSHOP PAPER

3/7/2019
- Created this file
- Added frontend/backend separation in Figure 1.
- Renamed frontend/backend to front-end/back-end
- Added evaluation results to Table 2
- Added description and formula for SELD metric.
- Abstract: changed percentage to generalize for evaluation set.
- Conclusion: changed percentage to generalize for evaluation set. Changed FR value from 9 to 10 to generalize.
- Results, conclusion: changed "our system improves" to "our system performs similar"

9/7/2019
- Removed SELD formula, added proper reference to journal paper for the metrics
- Fixed maximum STFT frequency in Table 1, rearranged for space
- Removed explanatory paragraph about frontend parameters (3.2)
- Removed \frac from Eq.4
- Added a comment about the naive approach of the association step
